UrbanCross: Enhancing Satellite Image-Text Retrieval with Cross-Domain Adaptation

Urbanization challenges underscore the necessity for effective satellite image-text retrieval methods to swiftly access specific information enriched with geographic semantics for urban applications. However, existing methods often overlook significant domain gaps across diverse urban landscapes, primarily focusing on enhancing retrieval performance within single domains. To tackle this issue, we present UrbanCross, a new framework for cross-domain satellite image-text retrieval. UrbanCross leverages a high-quality, cross-domain dataset enriched with extensive geo-tags from three countries to highlight domain diversity. It employs the Large Multimodal Model (LMM) for textual refinement and the Segment Anything Model (SAM) for visual augmentation, achieving a fine-grained alignment of images, segments and texts, yielding a 10% improvement in retrieval performance. Additionally, UrbanCross incorporates an adaptive curriculum-based source sampler and a weighted adversarial cross-domain fine-tuning module, progressively enhancing adaptability across various domains. Extensive experiments confirm UrbanCross's superior efficiency in retrieval and adaptation to new urban environments, demonstrating an average performance increase of 15% over its version without domain adaptation mechanisms, effectively bridging the domain gap.

==> contents/01introduction-raw.tex <==
\section{Introduction}

\begin{figure}[ht]
  \includegraphics[width=0.48\textwidth]{figures/intro.png}
    \caption{(a) highlights domain adaptation's role in differentiating solar power plants from residential houses across countries, while (b) illustrates geo-tags utility in enhancing semantic richness compared to visual intuition.}
  \label{fig: intro}
  \vspace{-1em}
\end{figure}

As global urbanization accelerates, the growing need for advanced tools in satellite imagery data retrieval has become increasingly prominent. Enriched with detailed geographic information, satellite imagery is essential for a broad range of applications including poverty assessment \cite{jean2016combining, jarry2021assessment}, crop yield prediction \cite{sabini2017understanding, rembold2013using}, and urban region profiling \cite{yan2023urban,hao2024urbanvlp}, etc. Crucially, satellite image-text retrieval, through modality alignment \cite{wang2016comprehensive, he2023end}, integrates visual and textual data, enhancing interpretation of urban complexities by correlating imagery with textual queries \cite{zou2024deep}. Research in this field is generally divided into two main paradigms \cite{zhou2023remote, abdullah2020towards}.

\begin{itemize}[leftmargin=*,itemsep=0.4ex,rightmargin=5pt,topsep=2pt]
    \item \emph{Content-based methods} concentrate on generating accurate captions for satellite images via generative models, converting image-text retrieval to a text-to-text task \cite{wang2020word, li2021recurrent}. For example, \citet{wang2020word} employ a word extractor integrated with a transformer-based sentence generator to improve the clarity of tags corresponding to the image, and \citet{li2021recurrent} utilize a recurrent attention and semantic gating mechanism to refine the semantic interpretation of captions.
    
    \item \emph{Embedding-based methods} leverage pre-trained encoders to align images and texts within a unified semantic space, ensuring better modal interaction \cite{lv2021fusion, yuan2021lightweight, yuan2022exploring}. For instance, \citet{yuan2022exploring} highlight salient features in images via visual self-attention module for enhanced representation learning, and \citet{cheng2021deep} focus on semantic alignment to increase retrieval accuracy. While Vision-Language Pre-training (VLP) like CLIP \cite{radford2021learning} have simplified cross-modal integration, their direct application to satellite images faces challenges including redundant objects and excessive background content. Hence, \citet{wang2022advancing} refine the visual encoder to excel with high-resolution images, and \citet{liu2023remoteclip} develop a pioneering vision-language model tailored for satellite imagery, boosting performance across various applications, including retrieval tasks.
\end{itemize}

Despite significant advancements, satellite image-text retrieval faces two primary challenges. \textbf{First}, the \textit{overlook of data distribution variations across different domains} often leads to the implicit assumption of uniformity in satellite image-text pairs across varied landscapes. For instance, in Figure \ref{fig: intro}(a), geographical differences, like the varying prevalence of solar power plants between Finland and Spain, due to distinct solar exposure levels, may result in the model trained on Finnish data incorrectly classifying Spanish solar plants as residential areas. This underscores the need for domain adaptation to ensure semantically equivalent feature alignment across geographies. \textbf{Second}, the \textit{poor quality of image-text pairs} may leads to misalignment between image and text. As shown in Figure \ref{fig: intro}(b), relying solely on visual features may lead to misinterpretation by visual encoders, underscoring the importance of incorporating geographic context for accuracy enhancement.

In response to these challenges, UrbanCross introduces a framework enhancing the embedding-based retrieval paradigm with integrated domain adaptation strategies, innovating at both data and model levels. \textbf{First}, UrbanCross \textit{integrates geo-tags with LMM} to generate visually rich and semantically accurate image captions. Additionally, it \textit{employs SAM for image segmentation} to extract fine-grained features, eliminating irrelevant elements and aligning these with corresponding text to enhance data quality across visual and language domains. \textbf{Second}, UrbanCross adopts a dual approach by combining an \textit{Adaptive Curriculum-based Source Sampler} with an \textit{Adversarial Cross-Domain Image-Text Fine-tuning module} to enhance domain adaptation capabilities. This integrated strategy ensures a seamless transition from simpler to more complex samples, applying nuanced weighting to align with domain-specific traits, thus effectively addressing the challenges posed by diverse data distributions across domains. All these methods establish UrbanCross as a pioneering solution in satellite image-text retrieval, setting new benchmarks for precision and effectiveness.	The key contributions of UrbanCross are summarized as follows:

\begin{itemize}[leftmargin=*,itemsep=0.4ex,rightmargin=5pt,topsep=2pt]
    \item \textbf{Data Augmentation}: Leveraging LMM and geo-tags, UrbanCross enriches textual descriptions of satellite images, enhancing contextual accuracy and semantic richness, and thereby creating high-quality image-text pairs.	
    \item \textbf{Fine-grained Modal Fusion}: UrbanCross employs SAM for detailed visual segmentation, removing irrelevant and detrimental features. This facilitates precise multi-modal fusion between segments, images, and texts, enhancing alignment.	
    \item \textbf{Domain Adaptation Integration}: Adaptive techniques are integrated through a curriculum-based source sampler and a weighted adversarial fine-tuning module, ensuring robust retrieval performance across diverse urban environments.
    \item \textbf{Extensive experiments}: Through extensive comparative and cross-country testing, UrbanCross has achieved a 10\% improvement in retrieval performance and a 15\% average boost over methods lacking domain adaptation.
\end{itemize}



==> supplementaries/01_Text_Generation_Analysis.tex <==
\section{Text Generation Analysis}

\subsection{LMM Selection Evaluation}
The efficacy of Large Multimodal Models (LMMs) in generating textual descriptions from images is pivotal to the success of cross-modal systems. To identify the most effective LMM for our research, we conducted a comparative analysis of prominent open-source models, as shown in Table \ref{table:lmms}. This evaluation centered on the \textit{PerceptionScore}, an innovative metric that quantifies the perceptual alignment of text with corresponding visual elements \cite{hao2024urbanvlp}. 

The \textit{PerceptionScore} integrates CLIPScore \cite{hessel-etal-2021-clipscore}, which leverages the robust zero-shot capabilities of CLIP \cite{radford2021learning} for text quality assessment, and the CycleScore.	This latter metric is designed to capture the visual recall of text, ensuring a comprehensive representation of all salient image details. The \textit{PerceptionScore} metric enables comprehensive evaluation of textual descriptions by focusing on the absence of specific image elements, thereby promoting precise alignment between the generated text and the image content.

\begin{table}[h]
\centering
\vspace{-1em}
\caption{Perception score of representative LMMs.}
\label{table:lmms}
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\captionsetup{labelformat=empty}
\begin{tabular}{c|c} 
\toprule
\rowcolor[rgb]{0.89,0.89,0.89} \textbf{Models} & \textbf{Average Generated Caption Scores} \\ 
\midrule
LLaVA-v1.5 \cite{liu2023improved} & 0.674 \\
mPLUG-Owl \cite{ye2023mplug} & 0.662 \\
LLaMA-Adapter V2 \cite{gao2023llama} & 0.698 \\
MiniGPTv2 \cite{chen2023minigpt} & 0.693 \\
ShareGPT4V \cite{chen2023sharegpt4v} & 0.714 \\ 
\hline
\textbf{InstructBLIP \cite{instructblip}} & \textbf{0.758} \\
\bottomrule
\end{tabular}
\vspace{-1em}
\end{table}

% % \vspace{-1em}
% \begin{gather}
% I'=\operatorname{SDXL}(I), CycleScore(I,I') = 1-\operatorname{MAE}(\operatorname{Seg}(I), \operatorname{Seg}(I')), \\
% PerceptionScore(I,T) = \frac{CLIPScore(I,T) + CycleScore(I,I')}{2}
% \end{gather}
% % \vspace{-1em}

Our experimental data, outlined in Table \ref{table:lmms}, indicates that InstructBLIP \cite{instructblip} surpasses other models with the highest \textit{PerceptionScore}. Consequently, we adopted InstructBLIP as our primary Image-to-Text model, due to its superior ability to generate perceptually coherent and contextually rich descriptions, a fundamental attribute for advancing text-image alignment in our UrbanCross framework.

\subsection{Prompt Design Comparison}
As shown in Figure \ref{fig: prompt_compare}, we conduct a comparison of various prompt designs aimed at providing a comprehensive overview of a specific location depicted in satellite imagery. We present two straightforward methods for prompt design: one involves prompting the LMM to generate its visual interpretation, while the other directs its attention toward geological features. However, both of these initial prompts lack the capacity to elicit nuanced information from the LMM. To address this limitation, we incorporate geo-tags information into our prompt, tailoring it to each individual satellite image. As a result, the location description becomes sufficiently detailed to discern diverse semantic nuances within the image itself.

\begin{figure}[h]
  \includegraphics[width=0.48\textwidth]{figures/caption.png}
  \caption{Prompt cases for location description generation.}
  \label{fig: prompt_compare}
  \vspace{-1em}
\end{figure}

\subsection{LMM Limitation Analysis}
As illustrated in Figure \ref{fig: lmm_bad_example}, our comprehensive analysis identifies specific scenarios where the Large Multimodal Models (LMMs) may exhibit suboptimal performance in generating text. This detailed investigation is designed to deepen our understanding of the LMM's capabilities as well as its limitations. Within this context, we have pinpointed three distinct scenarios that illustrate these challenges.

\begin{figure}[h]
  % \vspace{-1em}
  \includegraphics[width=0.48\textwidth]{figures/basecase.png}
    \caption{Bad examples of geo-tags enhanced text description generated by InstructBLIP.}
  \label{fig: lmm_bad_example}
  \vspace{-1em}
\end{figure}

\begin{itemize}[left=0pt]
    \item \textbf{Case 1}. When the Title Multi Objects contain elements outside the LMM’s pretraining data (e.g., "tracktype is grade2"), there is a risk of generating nonsensical descriptions.
    \item \textbf{Case 2}: When a term within the Title Multi Objects is polysemous (e.g., "driving range"), the LMM may misinterpret its meaning, resulting in incorrect text generation.
    \item \textbf{Case 3}: If the satellite image itself presents complexities that are difficult for human interpretation, particularly when accompanied by misleading geo-tags information, the resultant descriptions can be significantly degraded.
\end{itemize}


The causes of the aforementioned issues can be summarized as follows. Firstly, certain details in satellite images pose inherent challenges for human perception. Additionally, there is the issue of "hallucination" within the LMM itself, constrained by the capacity limitations of multimodal foundational models.




==> supplementaries/02_Image_Segmentation_Analysis.tex <==
\section{Image Segmentation Analysis}

\subsection{Image Segmentation and Text Enhancement}
The integration of image segmentation and geo-tags enrichment is essential for generating semantically rich text descriptions that align precisely with visual data. Figure \ref{fig: segment} presents a set of illustrative examples demonstrating this intricate interplay. In the top image, we observe a school area, where segmentation and corresponding geo-tags annotations such as "natural: scrub", "building: school", and "leisure: park" provide a detailed textual narrative. This enriching process allows for the precise capture of the surrounding environment, highlighting not just the main amenity but also peripheral elements such as adjacent roads and recreational areas.

Similarly, the bottom image showcases a healthcare facility marked by geo-tags indicating a "healthcare: laboratory" and "leisure: pitch", offering valuable insights into the facility's functionality and layout. These geo-tags are instrumental in guiding the segmentation algorithm to prioritize and detail salient features within the scene, such as parking amenities and service roads, which are pivotal for a comprehensive understanding of the landscape.

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.48\textwidth]{figures/segment.png}
  \vspace{-1em}
  \caption{Illustrative examples of our image segments and geo-tags enhanced descriptions.}
  \vspace{-1em}
  \label{fig: segment}
\end{figure}

By integrating geo-tags information, we not only refine the image segmentation but also enable the generation of text that captures a more granular and accurate depiction of the scene. This synergy between visual segmentation and textual enrichment is particularly evident when dealing with complex scenes where multiple objects or features must be precisely identified and described.

However, our methodology extends beyond simple annotation of images with geo-tags. It involves an iterative refinement where image segmentation informs the geo-tag-based text generation, and vice versa, leading to a fine-grained alignment that is greater than the sum of its parts. Such alignment is crucial for applications requiring detailed and context-aware descriptions of geographical spaces, as it allows for a nuanced interpretation of the environment, which is critical for accurate satellite image-text retrieval tasks.

\subsection{Fine-tuning Segmentation Parameters}
Our methodical calibration of the image segmentation process has conclusively established that six segments (\textit{num\_seg} = 6) provide the optimal representation of scenes for our modeling purposes. This specific number of segments was meticulously selected to adeptly capture the inherent complexity of diverse landscapes while avoiding the overburdening of the model with extraneous, non-essential details. The solid rationale behind this particular parameter choice is vividly demonstrated and well-supported by the statistical distributions, which are thoroughly illustrated in Figure \ref{fig: count_statistics}.

\begin{figure}[!h]
  \vspace{-1em}
  \centering
  \includegraphics[width=0.48\textwidth]{figures/count_statistics.pdf}
  \caption{Statistical distribution of tag count and word count of descriptions in our dataset, illustrating the optimal balance of information richness and brevity.}
  \vspace{-1em}
  \label{fig: count_statistics}
\end{figure}

The histogram on the left displays the frequency distribution of tag counts across our dataset. The majority of images have a tag count that clusters between four and ten, with a peak at six. This peak indicates that six tags often provide enough information to describe the essential elements of a scene without introducing noise through over-segmentation. The histogram on the right complements this finding by showing the word count distribution of the corresponding text descriptions. The majority of descriptions average approximately 54 words, achieving a balance between conciseness and detail necessary to comprehensively represent the scene for algorithmic processing and user interpretation.

This dual analysis of tag and word count distributions allows us to tailor our segmentation to align closely with the amount of detail that can be effectively described in texts, optimizing both the accuracy of image descriptions and the efficiency of our model. This fine-tuning ensures that each segment adds meaningful information to the generated description, facilitating a high level of detail in the semantic understanding of the scene, which is crucial for tasks such as image-text retrieval and scene comprehension.

\subsection{Future Segmentation Challenges}
While current segmentation approaches yield substantial improvements in text-image alignment, several challenges remain. These include poor segmentation performance for small objects, a lack of quantified metrics for assessing text quality, and the absence of an automatic refinement mechanism for the segmentation process. Addressing these issues will be crucial for future advancements. In subsequent iterations, tags could play a more pivotal role in guiding the joint training of image-text pairs \cite{huang2024tagtext}. Moreover, the adoption of a Chain-of-Thought mechanism \cite{feng2024towards}, which leverages feedback based on segmentation ratios, could enhance text quality further. These strategies offer promising avenues for improving the functionality and efficiency of our segmentation techniques.


==> supplementaries/03_Geo-Tags_Analysis.tex <==
\begin{figure*}[t!]
  \centering
  \includegraphics[width=1\textwidth]{figures/geotag.pdf}
  \vspace{-1em}
  \caption{Geo-Tags Word Cloud: Visualizing the Most Frequent Tags for Spain (a), Germany (b), and Finland (c); and Geo-Tags Clusters: Spatial Distribution Based on PCA for Spain (e), Germany (f), and Finland (g) across three countries.}
  \vspace{-1em}
  \label{fig: geotag}
\end{figure*}

% The clustering process involves a multi-step method where the frequency of geo-tags is first computed from the imagery, and a high-dimensional vector space is constructed. This space is then reduced to two principal components via PCA, capturing the most significant variances among the geo-tags. The clustering algorithm then divides these tags into coherent clusters, each distinguished by a unique color.



\section{Geo-Tags Analysis}
\subsection{Geo-Tags Distribution and Cluster Insights}
In exploring geospatial metadata, geo-tags serve as critical tools for extracting geographical semantics embedded within satellite imagery. This analysis employs frequency analysis of geo-tags sourced from satellite images across three distinct European regions: Finland, Germany, and Spain. Utilizing word clouds and PCA clustering, this study visually represents the distribution and frequency of these tags, thereby highlighting the most prominent geographical features captured within the imagery.

Word clouds and PCA clustering diagrams provide dual modalities for in-depth visual analysis. Word clouds are particularly effective for quickly identifying the most frequent and prominent geo-tags, with larger font sizes indicating higher frequencies. This visualization technique is augmented by PCA clustering, which groups geo-tags based on the similarity of their occurrences across various images, revealing underlying patterns that may not be immediately evident from the word clouds alone.

For instance, word clouds for Finland, Germany, and Spain showcase a distinct predominance of tags such as "natural", "building", and "waterway", amongst others. However, the PCA clustering diagrams further elucidate the relationships between these tags. In the case of Finland, the PCA clustering diagram shows that geo-tags associated with "piste:type" and "winter\_service" cluster together separately from common tags, highlighting the distinctive winter sports environment in the area.

The clustering technique used in this analysis involves a multi-step process. Initially, the frequency of geo-tags is computed from the dataset, and a high-dimensional vector space is created. This space is then simplified to two principal components through PCA, capturing the most significant variances among the geo-tags. Subsequently, the clustering algorithm subsequently divides these tags into coherent clusters, each marked by a unique color.

\subsection{Semantic Insights of Geo-Tags}
The insights from the word cloud and PCA clustering analyses significantly enhance our understanding of image-text alignment in cross-modal retrieval tasks. Specifically, PCA clustering illustrates the semantic proximity of geo-tags within their clusters, indicating potential shared functionalities or relationships. These insights not only emphasize the diverse geographical semantics inherent to the studied countries but also have profound implications for cross-modal retrieval tasks.

By leveraging clustering insights, searches for "recreational areas" could, for instance, pull images tagged with "leisure", "park", and "natural", knowing these tags share semantic relationships.

In summary, the frequency and cluster analysis of geo-tags not only lay a foundational layer for semantic comprehension but also illustrate distinct geographical semantics across different countries, which is essential for enhancing cross-modal retrieval tasks. The refined analytical methods in this study pave the way for extracting more detailed and context-rich insights from geo-tagged data, enriching the narratives that satellite imagery can offer.
